Proxion: Uncovering Hidden Proxy Smart Contracts for Finding Collision Vulnerabilities in Ethereum

The proxy design pattern allows Ethereum smart contracts to be simultaneously immutable and upgradeable, in which an original contract is split into a proxy contract containing the data storage and a logic contract containing the implementation logic. This architecture is known to have security issues, namely function collisions and storage collisions between the proxy and logic contracts, and has been exploited in real-world incidents to steal users' millions of dollars worth of digital assets. In response to this concern, several previous works have sought to identify proxy contracts in Ethereum and detect their collisions. However, they all fell short due to their limited coverage, often restricting analysis to only contracts with available source code or past transactions. To bridge this gap, we present Proxion, an automated cross-contract analyzer that identifies all proxy smart contracts and their collisions in Ethereum. What sets Proxion apart is its ability to analyze hidden smart contracts that lack both source code and past transactions. Equipped with various techniques to enhance efficiency and accuracy, Proxion outperforms the state-of-the-art tools, notably identifying millions more proxy contracts and thousands of unreported collisions. We apply Proxion to analyze over 36 million alive contracts from 2015 to 2023, revealing that 54.2% of them are proxy contracts, and about 1.5 million contracts exhibit at least one collision issue.

==> sections/implementation.tex <==
\section{Implementation}
\label{sec:implementation}

This section presents the detailed implementation of \codename, including a disassembler for smart contract bytecode (\S\ref{subsec:deassembler}), an EVM emulator (\S\ref{subsec:evm-emulator}), and the collisions detector (\S\ref{subsec:collision-detector}).
A prototype of \codename is accessible at {\em \url{https://github.com/Proxion-anonymous/Proxion}}.

\subsection{Disassembling Smart Contracts}
\label{subsec:deassembler}

To check if a smart contract is a proxy, \codename first disassembles its bytecode into opcodes. 
We implement this disassembler component of \codename based on Octopus, an open-source security analysis framework that is capable of translating contract bytecode into assembly representation (e.g., opcodes and operands)~\cite{octopus}. 
Particularly, we extend Octopus so that it covers recently introduced opcodes in Ethereum, such as {\tt CALL}, {\tt DELEGATECALL}, {\tt CREATE}, and {\tt CREATE2}.
This is easily achievable since the opcodes have fixed corresponding bytes.


\subsection{Emulating EVM}
\label{subsec:evm-emulator}

Given a contract containing \delegate opcodes, \codename emulates its execution in the EVM with a generated transaction and observes the memory, stack, and storage of each instruction. 
Here, we again extend Octopus to implement our EVM emulator. 

Specifically, our EVM emulator can also handle opcodes that have values depending on the state of the blockchain.
For example, to support the {\tt NUMBER} opcode that pushes the current block's number to the EVM stack, we use the values from the latest block on the blockchain since all alive contracts are supposed to be executable at any block's numbers.
Similarly, we use the values in the latest block for the {\tt BLOCKHASH}, {\tt DIFFICULTY}, {\tt GASLIMIT}, {\tt TIMESTAMP}, and {\tt GASPRICE} opcodes. 
We also assign fixed values for a few other opcodes, such as {\tt CHAINID}, {\tt BASEFEE}, and {\tt COINBASE}, using the most probable values (e.g., the chain ID of Ethereum's mainnet is 1).
Adding these blockchain-related opcodes makes the EVM emulator more complete (e.g., with fewer runtime errors when encountering them).
% and does not affect the emulation of delegate calls (see below) since no observed contract containing them and the \delegate opcode simultaneously.

Moreover, we implement our EVM emulator to support {\tt CALL} and \delegate opcodes that specifically call another contract and obtain the execution results before proceeding. 
To do so, we create two EVM emulator instances, one for the caller and another for the callee, and copy the results back from the callee to the stack of the caller instance to simulate the function returning.

For the opcodes that place bytecode on Ethereum at a smart-contract address (e.g., \texttt{CREATE} and \texttt{CREATE2}), we use a fixed address to ensure that we can retrieve the exact address of a newly created contract.
If our EVM emulator encounters this fixed address, we treat it like a normal smart contract. 
This method is acceptable because of the negligible probability of address collision (e.g., only 1 out of $2^{160}$ in Ethereum).

\subsection{Finding collisions}
\label{subsec:collision-detector}

Once the proxy contract and all its logic contracts are found, \name first uses Etherscan~\cite{etherscan}, a popular Ethereum explorer, to retrieve their source code. 
To ensure a consistent format for the contract source code, we also implement a parser to extract the source code returned by the Etherscan APIs, which can be in dictionary and array structures. 

Thereafter, \codename implements a static analyzer based on Slither~\cite{feist2019slither} to detect function and storage collisions. 
Particularly, we generate a list of both contracts' storage variables, including their types and names.
Then, we compare them one by one to spot any different types or names. 
We ignore the storage slots that are not used by both contracts (cf. Section~\ref{subsec:checking-collision}).
Regarding function collisions, we generate two lists of function signatures for both contracts. 
If these two lists intersect, we consider the two contracts collide. 

To speed up the collision detection in a large dataset, \codename also groups contracts based on their bytecode hash. 
That is, these contracts are exactly the same, albeit being deployed to different addresses.

==> sections/table-02.tex <==
\begin{table*}[ht] 
\caption{Number and percentage of contracts of each type in different datasets.}
\centering
\begin{adjustbox}{width=\textwidth}
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
     \hline
     \multicolumn{2}{|c|}{} & \multicolumn{7}{c|}{\textbf{Dataset}} \\
     \cline{3-9}
     \multicolumn{2}{|c|}{\textbf{Type}} & 2017 & 2018 & 2019 & 2020 & 2021 & 2022 & 2023\\
     \hline
     \multicolumn{2}{|c|}{proxy} & 80 (1.25\%)& 1,936 (1.71\%) & 1,062 (1.16\%) & 13,548 (16.48\%) & 31,560 (34.46\%) & 101,398 (88.71\%) & 26248 (60.94\%) \\
     \hline
     \multirow{3}{*}{non-proxy} & no delegatecall & 6,335 (98.74\%) & 110,684 (97.7\%) & 90,762 (98.72\%) & 68,328 (83.1\%) & 59,698 (65.18\%) & 12,775 (11.18\%) & 12879 (29.90\%) \\
        \cline{2-9}
        & delegate call & 0 (0\%) & 655 (0.58\%) & 106 (0.11\%) & 319 (0.39\%) & 309 (0.34\%) & 112 (0.1\%) & 3895 (9.04\%)\\
        \cline{2-9}
        & contract error & 1 (0.01\%) & 6 (0.01\%) & 10 (0.01\%) & 23 (0.03\%) & 19 (0.02\%) & 16 (0.01\%) & 53 (0.12\%)\\
     \hline
     \hline
     \multicolumn{2}{|c|}{\textbf{Total}} & 6,416 & 113,281 & 91,940 & 82,218 & 91,586 & 114,301 & 43,075\\
    \hline
    \end{tabular}
\end{adjustbox}
\label{delegate_table}
\end{table*}
